Ultracold Atoms in 1D Optical Lattices: Mean Field, Quantum Field, Computation, and Soliton Formation

In this work, we highlight the correspondence between two descriptions of a system of ultracold bosons in a one-dimensional optical lattice potential: (1) the discrete nonlinear Schr\"{o}dinger equation, a discrete mean-field theory, and (2) the Bose-Hubbard Hamiltonian, a discrete quantum-field theory. The former is recovered from the latter in the limit of a product of local coherent states. Using a truncated form of these mean-field states as initial conditions, we build quantum analogs to the dark soliton solutions of the discrete nonlinear Schr\"{o}dinger equation and investigate their dynamical properties in the Bose-Hubbard Hamiltonian. We also discuss specifics of the numerical methods employed for both our mean-field and quantum calculations, where in the latter case we use the time-evolving block decimation algorithm due to Vidal.

==> CHANGES <==
Changes from elsart 2.19 to 2.20
================================

Enable \tableofcontents at the end of the frontmatter
Suppress linenumbering in the frontmatter
Correct an error in the \collab command
Define \@ptsize to report the point size
Add \endNoHyper to \endfrontmatter
Change \let to \def in \endfigure, \endtable and \endalgorithm commands

Changes from elsart 2.18 to 2.19
================================

2006-05-01: added narrowdisplay option
2006-05-01: added draft and final option
2006-05-01: added \ensuremath around \ell in \@alph (suggested by
			Alik Widge)
2006-05-01: added \cal and \mit as alternatives for \mathcal and
			\mathnormal
2006-05-01, in \collab@fmt: added check for the presence of a
			footnote symbol
2001-02-22, in \collab@arg: \first@collab has been replaced with
			\first@author
2001-02-22, in \ead@au: changed \edef to \def
2001-12-14, in \collapse@citex: added code to remove leading spaces
			on cite key, from ltbibl

Changed files July 2006
=======================

Updated: elsart.cls.

New: elsart1p.cls, elsart3p.cls, elsart5p.cls.

Removed: elsart.sty, elsart12.sty. These are outdated.

Rewritten: instructions-harv.pdf, instructions-num.pdf. These replace
model-harv.pdf and model-num.pdf.

Removed: instraut. These instructions are outdated.

Modified: template-harv.tex, template-num.tex. The lineno package was
added.

